2D Thin obstacle problem with data at infinity

In this paper, we consider the thin obstacle problem in $\mathbb{R}^2$ with data at infinity. We first prove the existence and uniqueness of it. Then we show that its symmetric solutions are actually half-space solutions. Our results are needed when classifying the half-space $(2k-\frac{1}{2})$-homogeneous solutions to the thin obstacle problems in $\mathbb{R}^3$. It is a generalization of one part of Savin-Yu's work \cite{savin2021halfspace} on classifying the half-space $\frac{7}{2}$-homogeneous solutions.

==> bib1.tex <==
@book{gilbarg2015elliptic,
  title={Elliptic partial differential equations of second order},
  author={Gilbarg, David and Trudinger, Neil S},
  year={2015},
  publisher={springer}
}

@book{evans10,
	added-at = {2015-07-29T08:37:26.000+0200},
	address = {Providence, R.I.},
	author = {Evans, Lawrence C.},
	biburl = {https://www.bibsonomy.org/bibtex/2f5b120723ea78913e7e700ddd1a99301/ytyoun},
	interhash = {59982ce44cc43813ccb14c0d647a59ee},
	intrahash = {f5b120723ea78913e7e700ddd1a99301},
	isbn = {9780821849743 0821849743},
	keywords = {partial.differential.equations pde textbook},
	publisher = {American Mathematical Society},
	refid = {465190110},
	timestamp = {2015-07-29T08:37:26.000+0200},
	title = {Partial differential equations},
	year = 2010
}

